Weak regularization by degenerate L\'evy noise and its applications

After a general introduction about the regularization by noise phenomenon in the degenerate setting, the first part of this PhD thesis focuses at establishing the Schauder estimates, a useful analytical tool to prove also the well-posedness of stochastic differential equations (SDEs), for two different classes of Kolmogorov equations under a weak H\"ormander-like condition, whose coefficients lie in suitable anisotropic H\"older spaces with multi-indices of regularity. The first class considers a nonlinear system controlled by a symmetric stable operator acting only on some components. Our method of proof relies on a perturbative approach based on forward parametrix expansions through Duhamel-type formulas. Due to the low regularizing properties given by the degenerate setting, we also exploit some controls on Besov norms, in order to deal with the non-linear perturbation. As an extension of the first one, we also present Schauder estimates associated with a degenerate Ornstein-Uhlenbeck operator driven by a larger class of stable-like operators, like the relativistic or the Lamperti stable one. Exploiting a backward parametrix approach, the second part of this work aims at establishing the weak well-posedness for a degenerate chain of SDEs driven by the same class of stable-like processes, under the assumptions of the minimal H\"older regularity on the coefficients. As a by-product of our method, we also present Krylov-type estimates of independent interest for the associated canonical process. Finally, we show through suitable counter-examples the existence of an (almost) sharp threshold on the regularity exponents ensuring the weak well-posedness for the SDE. In connection with some possible applications to kinetic dynamics with friction, we conclude by investigating the stability of second-order perturbations for degenerate Kolmogorov operators in Lp and H\"older norms.

==> preamble.tex <==

\usepackage[T1]{fontenc}
\usepackage{amsthm}
\usepackage{tikz}
\usepackage{eucal}
\usepackage{dsfont}
\usepackage{mathrsfs}
\usepackage{stmaryrd}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{fancyhdr}
\usepackage{amssymb}
\usepackage{xcolor}
\definecolor{Prune}{RGB}{99,0,60}
\usepackage{mdframed}
\usepackage{multirow} %% Pour mettre un texte sur plusieurs rangées
\usepackage{multicol} %% Pour mettre un texte sur plusieurs colonnes
\usepackage{scrextend} %Forcer la 4eme  de couverture en page pair
\usepackage{tikz}
\usepackage{graphicx}
\usepackage[absolute]{textpos}
\usepackage{colortbl}
\usepackage{array}
\RequirePackage{geometry}% That nicely create a one-page template
%\geometry{textheight=100ex,textwidth=40em,top=100pt,headheight=30pt,headsep=30pt,inner=80pt}
\usepackage{geometry}
\usepackage{type1ec}
\usepackage{parskip}
\usepackage[final]{microtype}
\usepackage{lmodern}
\usepackage{textcomp}
\usepackage{pict2e}
\usepackage{enumitem}
\usepackage{hyperref}
\usepackage[nodayofweek]{datetime}
\usepackage{comment}
\usepackage{eepic}
\usepackage[italian,english,french]{babel}


\hypersetup{            pdfpagemode={UseOutlines},            bookmarksopen,               pdfstartview={FitH},                  colorlinks,                     linkcolor={black},                 citecolor={black},                  urlcolor={black}                               }

\fancypagestyle{plain}{%
  \fancyhf{}%
  \fancyfoot[LE,RO]{\thepage}%
  \renewcommand{\headrulewidth}{0pt}% Line at the header invisible
  \renewcommand{\footrulewidth}{0.5pt}% Line at the footer visible
}

\newcommand{\red}{\textcolor{red}}
\newcommand{\TheSubDate}{\monthyear \formatdate{04}{09}{2019}}
\newdateformat{monthyear}{\monthname[\THEMONTH], \THEYEAR}% new date format

\newcommand{\letdash}[1]{$#1$\nobreakdash-\hspace{0pt}}% for n-element, k-transitive etc

%\renewcommand{\theequation}{\thesection.\arabic{equation}}

\newcommand{\Z}{\ensuremath{\mathbb{Z}}}% integers
\newcommand{\N}{\ensuremath{\mathbb{N}}}% natural numbers
\newcommand{\R}{\ensuremath{\mathbb{R}}}% real numbers
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}% rational numbers
%\newcommand{\C}{\ensuremath{\mathbb{C}}}% complex numbers
\newcommand{\F}{\ensuremath{\mathbb{F}}} %real/complex field

% Operators
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\di}{div}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\sym}{Sym}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\rank}{rank}


\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{teorema}[theorem]{Teorema}
\newtheorem{theoreme}[theorem]{Théorème}
\theoremstyle{definition}
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{definition}[theorem]{Definition}



\renewcommand{\theequation}{\arabic{equation}}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\newcommand{\mysection}{\setcounter{equation}{0} \section}

%\newtheorem*{notation}{Notation}


\renewcommand
        {\thefootnote}{\fnsymbol{footnote}}
        


